Flatness Improves Backbone Generalisation in Few-shot Classification

Deployment of deep neural networks in real-world settings typically requires adaptation to new tasks with few examples. Few-shot classification (FSC) provides a solution to this problem by leveraging pre-trained backbones for fast adaptation to new classes. However, approaches for multi-domain FSC typically result in complex pipelines aimed at information fusion and task-specific adaptation without consideration of the importance of backbone training. In this work, we introduce an effective strategy for backbone training and selection in multi-domain FSC by utilizing flatness-aware training and fine-tuning. Our work is theoretically grounded and empirically performs on par or better than state-of-the-art methods despite being simpler. Further, our results indicate that backbone training is crucial for good generalisation in FSC across different adaptation methods.

==> fig/tikz/theorem.tex <==

	\begin{tikzpicture}
	\begin{axis}[
			ylabel={Loss},
			xlabel={Parameter},
			ylabel style={black!20,yshift=1em,font=\bf},
			xlabel style={black!20,yshift=-1em,font=\bf},
			grid=none,ticks=none, % helpers
			%axis lines=center,
			axis line style={black!20,line width=2pt},
			y axis line style={xshift=-1em},
			x axis line style={yshift=-1em},    
			axis y line=left,
			axis x line=bottom,
			xmin=-.1, xmax=1.1,
			ymin=-1.5, ymax=0.30,
			width=.8\columnwidth,
			height=.4\columnwidth,
			scale only axis,
			clip=false
	]
	% Define knots for the spline
	%\addplot[black!70, line width=1pt, mark=none, mark options={fill=red}] plot[smooth, tension=.7] coordinates {
	%    (0.00,-0.00) (0.06,-0.03) (0.09,-0.21) (0.10,-0.67) (0.12,-1.00) (0.15,-0.92) (0.18,-0.53) (0.21,-0.24) (0.29,-0.13) (0.41,-0.10) (0.46,-0.24) (0.48,-0.59) (0.55,-0.74) (0.62,-0.78) (0.72,-0.73) (0.75,-0.62) (0.78,-0.32) (0.84,-0.16) (0.92,-0.13) (1.00,-0.13)
	%};
	
	\addplot [line width=1.2pt, black!80] plot[smooth, tension=.7]
	table {%
	0 0
	0.0101010101010101 -0.000823569863181403
	0.0202020202020202 -0.00331588553557946
	0.0303030303030303 -0.00750935614147493
	0.0404040404040404 -0.0134363908051486
	0.0505050505050505 -0.0211293986508812
	0.0606060606060606 -0.0306641433006384
	0.0707070707070707 -0.0570063153567238
	0.0808080808080808 -0.117805182037253
	0.0909090909090909 -0.227936321240684
	0.101010101010101 -0.695782180463137
	0.111111111111111 -0.918644214362372
	0.121212121212121 -0.999826738206799
	0.131313131313131 -0.986210976337434
	0.141414141414141 -0.955267319900841
	0.151515151515152 -0.911876597407846
	0.161616161616162 -0.801123013786986
	0.171717171717172 -0.643573365875997
	0.181818181818182 -0.509423943928018
	0.191919191919192 -0.38879038604917
	0.202020202020202 -0.285043437266984
	0.212121212121212 -0.234335338496154
	0.222222222222222 -0.209950719639143
	0.232323232323232 -0.189555064493318
	0.242424242424242 -0.172752045275581
	0.252525252525253 -0.159145334202832
	0.262626262626263 -0.148338603491972
	0.272727272727273 -0.139935525359904
	0.282828282828283 -0.133539772023528
	0.292929292929293 -0.128710618667826
	0.303030303030303 -0.124423082404986
	0.313131313131313 -0.120399951670086
	0.323232323232323 -0.116665467965361
	0.333333333333333 -0.113243872793044
	0.343434343434343 -0.11015940765537
	0.353535353535354 -0.107436314054573
	0.363636363636364 -0.105098833492887
	0.373737373737374 -0.103171207472546
	0.383838383838384 -0.101677677495785
	0.393939393939394 -0.100642485064838
	0.404040404040404 -0.100089871681939
	0.414141414141414 -0.101028236425457
	0.424242424242424 -0.111984312375717
	0.434343434343434 -0.134495652773804
	0.444444444444444 -0.168029511448771
	0.454545454545455 -0.212053142229671
	0.464646464646465 -0.298940067665668
	0.474747474747475 -0.522985325012205
	0.484848484848485 -0.610528778336563
	0.494949494949495 -0.646616065906381
	0.505050505050505 -0.674802818695802
	0.515151515151515 -0.696453364669944
	0.525252525252525 -0.712932031793924
	0.535353535353535 -0.725603148032859
	0.545454545454546 -0.735831041351867
	0.555555555555556 -0.74496432986388
	0.565656565656566 -0.753621822030749
	0.575757575757576 -0.761545662729496
	0.585858585858586 -0.768432219691885
	0.595959595959596 -0.773977860649683
	0.606060606060606 -0.777878953334653
	0.616161616161616 -0.779831865478561
	0.626262626262626 -0.77981088364321
	0.636363636363636 -0.778703713208328
	0.646464646464647 -0.776595979436062
	0.656565656565657 -0.773475931901874
	0.666666666666667 -0.769331820181226
	0.676767676767677 -0.764151893849583
	0.686868686868687 -0.757924402482405
	0.696969696969697 -0.750637595655157
	0.707070707070707 -0.7422797229433
	0.717171717171717 -0.732839033922298
	0.727272727272727 -0.716654161986677
	0.737373737373737 -0.68164001025456
	0.747474747474748 -0.633373591473344
	0.757575757575758 -0.555992605397294
	0.767676767676768 -0.433523043441717
	0.777777777777778 -0.332449953717644
	0.787878787878788 -0.286306193905233
	0.797979797979798 -0.248397678336675
	0.808080808080808 -0.216672366561663
	0.818181818181818 -0.191390196714345
	0.828282828282828 -0.172811106928863
	0.838383838383838 -0.161195035339362
	0.848484848484849 -0.154434883283003
	0.858585858585859 -0.148424613812072
	0.868686868686869 -0.1431448755774
	0.878787878787879 -0.138661367361308
	0.888888888888889 -0.135039787946118
	0.898989898989899 -0.13234583611415
	0.909090909090909 -0.130645210647727
	0.919191919191919 -0.130003610329169
	0.929292929292929 -0.13
	0.939393939393939 -0.13
	0.94949494949495 -0.13
	0.95959595959596 -0.13
	0.96969696969697 -0.13
	0.97979797979798 -0.13
	0.98989898989899 -0.13
	1 -0.13
	};
	
	\addplot [line width=1.2pt, ruiblue, opacity=0.5] plot[smooth, tension=.7]
	table {%
	0 0.1
    0.0101010101010101 0.0803806252738389
    0.0202020202020202 0.060950350887849
    0.0303030303030303 0.0417600424398612
    0.0404040404040404 0.0228605655277061
    0.0505050505050505 0.00430278574921483
    0.0606060606060606 -0.0138624312977819
    0.0707070707070707 -0.0315842200154532
    0.0808080808080808 -0.0488117148059682
    0.0909090909090909 -0.0654940500714961
    0.101010101010101 -0.081577079024718
    0.111111111111111 -0.0966661066308244
    0.121212121212121 -0.110630434156952
    0.131313131313131 -0.123634159257868
    0.141414141414141 -0.135841379588339
    0.151515151515152 -0.147416192803131
    0.161616161616162 -0.158522696557012
    0.171717171717172 -0.169324988504749
    0.181818181818182 -0.179987166301108
    0.191919191919192 -0.190673327600855
    0.202020202020202 -0.201547570058759
    0.212121212121212 -0.212773991329585
    0.222222222222222 -0.2245166890681
    0.232323232323232 -0.236939760929072
    0.242424242424242 -0.250207304567267
    0.252525252525253 -0.264483417637452
    0.262626262626263 -0.279932197794393
    0.272727272727273 -0.296717742692858
    0.282828282828283 -0.315004149987613
    0.292929292929293 -0.334955517333425
    0.303030303030303 -0.357245452980215
    0.313131313131313 -0.389616845393791
    0.323232323232323 -0.433507528510542
    0.333333333333333 -0.487447916666667
    0.343434343434343 -0.549968424198366
    0.353535353535354 -0.619599465441838
    0.363636363636364 -0.694871454733283
    0.373737373737374 -0.774314806408901
    0.383838383838384 -0.85645993480489
    0.393939393939394 -0.939837254257451
    0.404040404040404 -1.02297717910278
    0.414141414141414 -1.10441012367708
    0.424242424242424 -1.18266650231655
    0.434343434343434 -1.25627672935739
    0.444444444444444 -1.3237712191358
    0.454545454545455 -1.38368038598798
    0.464646464646465 -1.43453464425012
    0.474747474747475 -1.47486440825843
    0.484848484848485 -1.50320009234911
    0.494949494949495 -1.51807211085835
    0.505050505050505 -1.51896560051519
    0.515151515151515 -1.51093189867983
    0.525252525252525 -1.49548164645272
    0.535353535353535 -1.47325882794891
    0.545454545454546 -1.44490742728346
    0.555555555555556 -1.41107142857143
    0.565656565656566 -1.37239481592787
    0.575757575757576 -1.32952157346785
    0.585858585858586 -1.28309568530643
    0.595959595959596 -1.23376113555866
    0.606060606060606 -1.18216190833959
    0.616161616161616 -1.1289419877643
    0.626262626262626 -1.07474535794784
    0.636363636363636 -1.02021600300526
    0.646464646464647 -0.965997907051626
    0.656565656565657 -0.912735054201996
    0.666666666666667 -0.861071428571428
    0.676767676767677 -0.811651014274981
    0.686868686868687 -0.765117795427712
    0.696969696969697 -0.722115756144681
    0.707070707070707 -0.681641898671042
    0.717171717171717 -0.639432294757745
    0.727272727272727 -0.595552295548327
    0.737373737373737 -0.550365554094436
    0.747474747474748 -0.504235723447722
    0.757575757575758 -0.457526456659833
    0.767676767676768 -0.41060140678242
    0.777777777777778 -0.363824226867131
    0.787878787878788 -0.317558569965615
    0.797979797979798 -0.272168089129521
    0.808080808080808 -0.228016437410499
    0.818181818181818 -0.185467267860198
    0.828282828282828 -0.144884233530266
    0.838383838383838 -0.106630987472353
    0.848484848484849 -0.0710711827381085
    0.858585858585859 -0.0385684723791804
    0.868686868686869 -0.00948650944721902
    0.878787878787879 0.0158110530061273
    0.888888888888889 0.036960561929209
    0.898989898989899 0.0535983642703771
    0.909090909090909 0.0673393413721538
    0.919191919191919 0.0807584977965198
    0.929292929292929 0.0936101043529515
    0.939393939393939 0.105624161589713
    0.94949494949495 0.116530670055068
    0.95959595959596 0.126059630297281
    0.96969696969697 0.133941042864617
    0.97979797979798 0.139904908305339
    0.98989898989899 0.143681227167712
    1 0.145
	};
	
	% Local and global minima
	\node[fill=ruired,inner sep=1pt,circle] (sharpmin) at (axis cs: 0.121212121212121,-0.999826738206799) {};
	\node[fill=ruigreen,inner sep=1pt,circle] (flatmin) at (axis cs: 0.616161616161616,-0.779831865478561) {};
	\node[fill=blue,inner sep=1pt,circle] (gmin) at (axis cs: 0.505050505050505, -1.51896560051519) {};
	\node[fill=ruigreen,inner sep=1pt,circle] (flatattest) at (axis cs: 0.616161616161616, -1.1289419877643) {};
	
	% distance between sharp and flat

	\draw[line width=1pt,ruigreen] (0, -0.999826738206799) -- (sharpmin);
	\draw[line width=1pt,ruigreen] (0, -0.779831865478561) -- (flatmin);
	\draw[line width=1pt,ruigreen,->,-latex,shorten >=0.05cm,shorten <=.05cm] 
		($(0.01, -0.999826738206799) $) -- 
		node[midway,xshift=-1em,font=\scriptsize]{text1}
		($(0.01, -0.779831865478561) $);
%	\node[black,font=\scriptsize] at ($(sharpmin) + (axis direction cs:0,-.2)$) 
%		{Sharp minimum};
	
	% distance between test minimal and flat
	\draw[line width=1pt,gray,dashed] (flatmin) -- (flatattest);
	\draw[line width=1pt,ruiorange] (gmin) -- (0.9, -1.51896560051519);
	\draw[line width=1pt,ruiorange] (flatattest) --(0.9, -1.1289419877643);
	\draw[line width=1pt,ruiorange,->,-latex,shorten >=0.05cm,shorten <=.05cm] 
		($(0.85, -1.51896560051519) + (axis direction cs:.0,0)$) -- 
		node[midway,xshift=2em,font=\scriptsize]{text2}
		($(0.85, -1.1289419877643) + (axis direction cs:.0,0)$);
%	\node[black,font=\scriptsize] at ($(flatmin) + (axis direction cs:0,.15)$) 
%		{Flat minimum};
	
	% Other labels
	\node[ruiblue,opacity=.5,font=\scriptsize,anchor=west] at (axis cs: 0.9,.25) {Test (true)};
	\node[black!80,font=\scriptsize,anchor=west] at (axis cs: 0.9,-.25) {Train (emperical)};
	
	\end{axis}
	\end{tikzpicture}

==> table/bSAM_simple.tex <==
\begin{tabular}{l|ccccccc}
\toprule
{} &    Simple CNAPS     & Transductive CNAPS  &        SUR          &        URT          &        URL          &        TSA          &       b-SAM         \\\hline
 {\sc ilsvrc\_2012}  & $   56.03{\pm}1.11   $ & $   56.61{\pm}1.08   $ & $   55.09{\pm}1.09   $ & $   55.17{\pm}1.08   $ & $   55.65{\pm}1.07   $ & $   55.67{\pm}1.07   $ & $ \bf58.50{\pm}1.06  $ \\
   {\sc omniglot}    & $   91.45{\pm}0.62   $ & $   92.91{\pm}0.50   $ & $   94.38{\pm}0.44   $ & $   94.42{\pm}0.46   $ & $   94.76{\pm}0.41   $ & $ \bf95.03{\pm}0.41  $ & $   94.03{\pm}0.46   $ \\
   {\sc aircraft}    & $   80.90{\pm}0.73   $ & $   82.11{\pm}0.63   $ & $   87.68{\pm}0.47   $ & $   88.16{\pm}0.47   $ & $   89.57{\pm}0.45   $ & $   89.95{\pm}0.45   $ & $ \bf90.76{\pm}0.39  $ \\
  {\sc cu\_birds}    & $   75.10{\pm}0.86   $ & $   77.35{\pm}0.77   $ & $   72.28{\pm}0.92   $ & $   79.04{\pm}0.77   $ & $   81.51{\pm}0.69   $ & $   82.08{\pm}0.72   $ & $ \bf82.63{\pm}0.66  $ \\
     {\sc dtd}       & $   68.90{\pm}0.72   $ & $   68.76{\pm}0.73   $ & $   72.08{\pm}0.73   $ & $   73.05{\pm}0.67   $ & $   74.66{\pm}0.65   $ & $ \bf75.63{\pm}0.67  $ & $ \bf75.95{\pm}0.69  $ \\
  {\sc quickdraw}    & $   77.53{\pm}0.77   $ & $   78.74{\pm}0.67   $ & $   83.36{\pm}0.56   $ & $   83.51{\pm}0.56   $ & $   82.42{\pm}0.61   $ & $   82.33{\pm}0.62   $ & $ \bf83.87{\pm}0.57  $ \\
    {\sc fungi}      & $   48.07{\pm}1.10   $ & $   48.39{\pm}1.12   $ & $   68.68{\pm}0.97   $ & $   68.23{\pm}0.99   $ & $   68.44{\pm}0.98   $ & $   67.62{\pm}0.97   $ & $ \bf71.47{\pm}0.91  $ \\
 {\sc vgg\_flower}   & $   91.45{\pm}0.52   $ & $   92.25{\pm}0.45   $ & $   87.11{\pm}0.52   $ & $   90.09{\pm}0.46   $ & $   91.55{\pm}0.44   $ & $ \bf92.90{\pm}0.43  $ & $   92.06{\pm}0.41   $ \\
\midrule
{\sc traffic\_sign}  & $   58.33{\pm}1.03   $ & $   56.83{\pm}1.13   $ & $   45.33{\pm}1.02   $ & $   47.11{\pm}1.02   $ & $   60.15{\pm}1.18   $ & $ \bf81.51{\pm}0.97  $ & $   80.89{\pm}0.92   $ \\
    {\sc mscoco}     & $   48.79{\pm}1.09   $ & $   50.89{\pm}1.05   $ & $   50.41{\pm}1.03   $ & $   50.15{\pm}1.03   $ & $   52.82{\pm}1.01   $ & $   53.98{\pm}1.07   $ & $ \bf55.86{\pm}1.03  $ \\
    {\sc mnist}      & $   93.81{\pm}0.42   $ & $   95.13{\pm}0.30   $ & $   94.71{\pm}0.42   $ & $   88.89{\pm}0.48   $ & $   94.84{\pm}0.42   $ & $   96.65{\pm}0.37   $ & $ \bf97.46{\pm}0.30  $ \\
   {\sc cifar10}     & $   71.75{\pm}0.76   $ & $   72.60{\pm}0.68   $ & $   68.76{\pm}0.76   $ & $   64.50{\pm}0.75   $ & $   69.93{\pm}0.74   $ & $   78.93{\pm}0.77   $ & $ \bf80.02{\pm}0.71  $ \\
   {\sc cifar100}    & $   61.62{\pm}1.05   $ & $   62.35{\pm}1.02   $ & $   59.32{\pm}1.05   $ & $   55.85{\pm}1.07   $ & $   61.58{\pm}1.09   $ & $   70.11{\pm}1.00   $ & $ \bf71.94{\pm}0.93  $ \\
\midrule
    Average Seen     & $73.68$ & $74.64$ & $77.58$ & $78.96$ & $79.82$ & $80.15$ & $81.16$ \\
   Average Unseen    & $66.86$ & $67.56$ & $63.71$ & $61.30$ & $67.86$ & $76.24$ & $77.23$ \\
\bottomrule\end{tabular}


==> table/sdl_compare.tex <==
\begin{tabular}{l|cc|cc}
\toprule
{} &      ERM sur        &      SAM sur        &      ERM tsa        &      SAM tsa        \\\hline
 {\sc ilsvrc\_2012}  & $   55.09{\pm}1.09   $ & $   56.25{\pm}1.08   $ & $   56.74{\pm}1.08   $ & $   58.50{\pm}1.06   $ \\
   {\sc omniglot}    & $   94.38{\pm}0.44   $ & $   93.95{\pm}0.46   $ & $   94.64{\pm}0.43   $ & $   94.19{\pm}0.46   $ \\
   {\sc aircraft}    & $   87.68{\pm}0.47   $ & $   87.74{\pm}0.45   $ & $   88.24{\pm}0.45   $ & $   88.68{\pm}0.43   $ \\
  {\sc cu\_birds}    & $   72.28{\pm}0.92   $ & $   72.68{\pm}0.82   $ & $   70.57{\pm}0.86   $ & $   73.19{\pm}0.83   $ \\
     {\sc dtd}       & $   72.08{\pm}0.73   $ & $   73.08{\pm}0.73   $ & $   61.33{\pm}0.71   $ & $   62.73{\pm}0.76   $ \\
  {\sc quickdraw}    & $   83.36{\pm}0.56   $ & $   83.75{\pm}0.56   $ & $   83.64{\pm}0.58   $ & $   84.00{\pm}0.58   $ \\
    {\sc fungi}      & $   68.68{\pm}0.97   $ & $   70.67{\pm}0.95   $ & $   68.45{\pm}0.96   $ & $   70.54{\pm}0.92   $ \\
 {\sc vgg\_flower}   & $   87.11{\pm}0.52   $ & $   86.41{\pm}0.54   $ & $   84.28{\pm}0.58   $ & $   83.48{\pm}0.62   $ \\
\midrule
{\sc traffic\_sign}  & $   45.33{\pm}1.02   $ & $   44.06{\pm}1.15   $ & $   80.71{\pm}0.97   $ & $   80.88{\pm}0.92   $ \\
    {\sc mscoco}     & $   50.41{\pm}1.03   $ & $   48.54{\pm}1.03   $ & $   56.07{\pm}1.05   $ & $   55.88{\pm}1.02   $ \\
    {\sc mnist}      & $   94.71{\pm}0.42   $ & $   95.52{\pm}0.30   $ & $   96.59{\pm}0.35   $ & $   97.29{\pm}0.31   $ \\
   {\sc cifar10}     & $   68.76{\pm}0.76   $ & $   68.94{\pm}0.94   $ & $   79.60{\pm}0.73   $ & $   80.04{\pm}0.71   $ \\
   {\sc cifar100}    & $   59.32{\pm}1.05   $ & $   61.20{\pm}1.09   $ & $   71.19{\pm}0.96   $ & $   71.95{\pm}0.93   $ \\
\midrule
    Average Seen     & $77.58$ & $78.07$ & $75.99$ & $76.91$ \\
   Average Unseen    & $63.71$ & $63.65$ & $76.83$ & $77.21$ \\
\bottomrule\end{tabular}

